Redefining Absent Keyphrases and their Effect on Retrieval Effectiveness

Neural keyphrase generation models have recently attracted much interest due to their ability to output absent keyphrases, that is, keyphrases that do not appear in the source text. In this paper, we discuss the usefulness of absent keyphrases from an Information Retrieval (IR) perspective, and show that the commonly drawn distinction between present and absent keyphrases is not made explicit enough. We introduce a finer-grained categorization scheme that sheds more light on the impact of absent keyphrases on scientific document retrieval. Under this scheme, we find that only a fraction (around 20%) of the words that make up keyphrases actually serves as document expansion, but that this small fraction of words is behind much of the gains observed in retrieval effectiveness. We also discuss how the proposed scheme can offer a new angle to evaluate the output of neural keyphrase generation models.

==> _attic/perf-kg-model.tex <==

\begin{table*}[!ht]
    \centering
    \begin{tabular}{ll|rrrr}
    \multicolumn{3}{c}{~} &
    \multicolumn{3}{c}{\small{$\lceil$ \hfill {\scriptsize absent keyphrases} \hfill $\rceil$}}
    \\
    \midrule
    \textbf{Model} & \textbf{Dataset} & \textbf{\%P} & \textbf{\%R} & \textbf{\%M} & \textbf{\%U} \\
    \midrule
        %CopyRNN
        seq2seq+copy
                 & KP20k    & 33.4 & 1.5 & 1.0 & 0.4 \\
                 & NTCIR1+2 & 28.5 & 0.1 & 0.1 & 0.0 \\
        \midrule
        %CorrRNN
        seq2seq+corr
                 & KP20k    & 29.3 & 1.5 & 0.7 & 0.3 \\
                 & NTCIR1+2 & 27.0 & 0.4 & 0.1 & 0.0 \\
        \midrule
        %catTGNet
        cat-seq2seq+tg
                 & KP20k    & 32.0 & 2.0 & 1.8 & 1.1 \\
                 & NTCIR1+2 & 18.4 & 0.5 & 0.5 & 0.3 \\
    \bottomrule
    \multicolumn{2}{c}{~} &
    \multicolumn{2}{c@{}}{\small{$\lfloor$ \hfill {\scriptsize term-weighting} \hfill $\rfloor$}} &
    \multicolumn{2}{c}{\small{$\lfloor$ \hfill {\scriptsize doc. expansion} \hfill $\rfloor$}}
    \end{tabular}
    \caption{Performance (f-score \@ 5)  according to \underline{P}resent, \underline{R}eordered, \underline{M}ixed and \underline{U}nseen keyphrases in model's output. \textcolor{purple}{C'est un très gros tableau, mais c'est juste pour le regarder.}}
    \label{tab:perf-kg-model}
\end{table*}

==> _attic/retrieval-results-models.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{ll|cc}
        \toprule
        \textbf{model} & \textbf{index} & \textbf{BM25} & \textbf{+RM3} \\
        %\cmidrule(lr){2-3} \cmidrule(lr){4-5}
        %~ & MAP & P10 & MAP & P10 \\
        \midrule

        & title+abstract   & 29.55 & 32.83 \\
\midrule
CopyRNN & All              & 31.71 & 34.40  \\
\cmidrule(lr){2-4}
CopyRNN & Present          & 31.71 & 34.01 \\
CopyRNN & Reordered        & 29.82 & 33.37 \\
CopyRNN & Mixed            & 29.69 & 33.22 \\
CopyRNN & Unseen           & 29.57 & 33.04 \\
\cmidrule(lr){2-4}
CopyRNN & Absent           & 29.86 & 33.51 \\
\cmidrule(lr){2-4}
CopyRNN & Highlight (P+R)  & 31.65 & 34.07 \\
CopyRNN & Expand (M+U)     & 29.64 & 33.29 \\

\midrule

CorrRNN & All              & 30.56 & 34.04 \\
\cmidrule(lr){2-4}
CorrRNN & Present          & 30.62 & 34.44 \\
CorrRNN & Reordered        & 29.46 & 32.56 \\
CorrRNN & Mixed            & 29.69 & 33.13 \\
CorrRNN & Unseen           & 29.55 & 32.80  \\
\cmidrule(lr){2-4}
CorrRNN & Absent           & 29.34 & 32.89 \\
\cmidrule(lr){2-4}
CorrRNN & Highlight (P+R)  & 30.54 & 34.25 \\
CorrRNN & Expand (M+U)     & 29.62 & 32.90  \\

\midrule

catTGNet & All             & 28.87 & 32.07 \\
\cmidrule(lr){2-4}
catTGNet & Present         & 29.83 & 33.91 \\
catTGNet & Reordered       & 29.46 & 32.78 \\
catTGNet & Mixed           & 29.70 & 32.86 \\
catTGNet & Unseen          & 28.82 & 31.41 \\
\cmidrule(lr){2-4}
catTGNet & Absent          & 28.67 & 30.59 \\
\cmidrule(lr){2-4}
catTGNet & Highlight (P+R) & 29.66 & 33.38 \\
catTGNet & Expand (M+U)    & 28.76 & 31.05 \\
         \bottomrule
    \end{tabular}
    \caption{Retrieval effectiveness (mAP) of BM25 and BM23+RM3 using various indexing configurations and models. Variants were computed using 10 best keyphrases of the output.}
    \label{tab:retrieval_results_models}
\end{table*} % 0.05

==> _attic/retrieval-results.tex <==
\begin{table}[ht!]
    \centering
    \begin{tabular}{l|cc||c}
        \toprule
        \textbf{index} & \textbf{BM25} & \textbf{+RM3} & \textbf{\#kp}\\
        %\cmidrule(lr){2-3} \cmidrule(lr){4-5}
        %~ & MAP & P10 & MAP & P10 \\
        \midrule
            title \& abstract   & 29.64 & 32.78 & -\\
        \cmidrule(lr){1-4}
            ~+~\underline{P}resent   & 30.74$^\dagger$ & 33.46 & 2.9 \\
            ~+~\underline{R}eordered & 29.79 & 33.39 & 0.4 \\ %C1
            ~+~\underline{M}ixed     & \textbf{30.86}$^\dagger$ & 33.86 & 0.8 \\ %C2
            ~+~\underline{U}nseen    & 29.68 & \textbf{33.92}$^\dagger$ & 0.7 \\ % C3
        \cmidrule(lr){1-4}
            ~+~Absent \scriptsize{(R+M+U)}    & 30.80 & 34.92$^\dagger$ & 1.9 \\ % abs
        \cmidrule(lr){1-4}
            ~+~Highlight \scriptsize{(P+R)}   & 30.64$^\dagger$ & 33.79 & 3.3 \\ % P+C1
            ~+~Expand \scriptsize{(M+U)}   & \textbf{30.88}$^\dagger$ & \textbf{34.34} & 1.5 \\ % C2+C3
         \cmidrule(lr){1-4}
            ~+~all \scriptsize{(P+R+M+U)}       & 31.92$^\dagger$ & 35.46$^\dagger$  & 4.8 \\
         \bottomrule
    \end{tabular}
    \caption{Retrieval effectiveness (mAP) of BM25 and BM23+RM3 using various indexing configurations. We also report the average number of keyphrases (\#kp). $\dagger$ indicates significance over title \& abstract indexing.}
    \label{tab:retrieval_results}
\end{table}

==> tables/changes.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|rrr|rrr}
        \toprule
        ~ & \multicolumn{3}{c}{BM25} & \multicolumn{3}{c}{+RM3} \\
        \textbf{index} & $-$ & $\approx$ & $+$ & $-$ & $\approx$ & $+$ \\
        \midrule
         T+A+K-pres  & 27 & 8 & 65 & 35 & 2 & 63 \\
         T+A+K-abs   & 39 & 12 & 49 & 31 & 4 & 65 \\
         T+A+K       & 24 & 6 & 69 & 20 & 2 & 78 \\
         \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:changes}
\end{table}

==> tables/comp-model-ir.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{lrrrrrr|rl}
    %\multicolumn{3}{c}{~} &
    %\multicolumn{3}{c}{\small{$\lceil$ \hfill {\scriptsize absent keyphrases} \hfill $\rceil$}}
    \\
    \midrule
     & & & & & & & & BM25+RM3 \\
    \textbf{Model} & \textbf{\#} & \textbf{\%P} & \textbf{\%R} & \textbf{\%M} & \textbf{\%U} & \textbf{\%uw} &  \textbf{F$@$5} & mAP {\small (cf.~32.83)} \\
    %\textbf{Model} & \textbf{\#} & \textbf{\%P} & \textbf{\%R} & \textbf{\%M} & \textbf{\%U} & \textbf{\%uw} &  \textbf{F$@$5} & \textbf{F$@$10} & \textbf{mAP$@$5} & \textbf{mAP$@$10} \\
    \midrule
        %ref            & 4.8 & 61.2 &  8.2 & 16.6 & 14.1 & 21.5 &    - &    - & \multicolumn{2}{c}{35.22} \\
        %seq2seq+copy   & 5.0 & 96.9 &  1.3 &  0.9 &  0.9 & 12.3 & 24.0 & 22.3 & 34.58 & 34.40 \\
        % seq2seq+corr  & 5.0 & 89.7 &  7.1 &  2.5 &  0.8 &  3.2 & 22.1 & 20.7 & 35.13 & 34.04 \\
        %cat-seq2seq+tg & 4.4 & 52.3 &  3.0 &  8.7 & 36.0 & 40.0 & 14.0 & 14.7 & 32.16 & 32.07 \\
                 
        ref
                 & 4.8 & 61.2 &  8.2 & 16.6 & 14.1 & 21.5 &    - & 35.22 \\
        seq2seq+copy
                 & 5.0 & 96.9 &  1.3 &  0.9 &  0.9 & 12.3 & 24.0 & 34.58 \\
         seq2seq+corr
                 & 5.0 & 89.7 &  7.1 &  2.5 &  0.8 &  3.2 & 22.1 & 35.13 \\
        cat-seq2seq+tg
                 & 4.4 & 52.3 &  3.0 &  8.7 & 36.0 & 40.0 & 14.0 & 32.16 \\
    \bottomrule
    %\multicolumn{2}{c}{~} &
    %\multicolumn{2}{c@{}}{\small{$\lfloor$ \hfill {\scriptsize term-weighting} \hfill $\rfloor$}} &
    %\multicolumn{2}{c}{\small{$\lfloor$ \hfill {\scriptsize doc. expansion} \hfill $\rfloor$}}
    \end{tabular}
    \caption{Number (\#) and proportion of \underline{P}resent, \underline{R}eordered, \underline{M}ixed and \underline{U}nseen keyphrases in model's top 5 output with NTCIR1+2. We also report the ratio of unique, unseen words in M+U keyphrases (\%uw).}
    \label{tab:perf-dist-model}
\end{table*}


==> tables/datasets.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{l|rrr|rrrr|r}
    \multicolumn{2}{c}{~} &
    \multicolumn{3}{c}{\small{$\lceil$ \hfill {\scriptsize absent keyphrases} \hfill $\rceil$}}
    \\
    \toprule
        \textbf{Dataset} &
        \textbf{\#D} &
        \textbf{\#Q} &
        \textbf{\#kps} &
        \textbf{\%P} &
        \textbf{\%R} &
        \textbf{\%M} &
        \textbf{\%U} &
        \textbf{\%uw} \\
    \midrule
     NTCIR-2 & 61.2 &  8.2 & 16.6 & 14.1 & 21.5 \\
     ACM-IR  & 53.6 & 11.7 & 19.3 & 15.4 & 13.4\\
     KP20k   & 60.2 &  9.5 & 15.4 & 15.0 & 22.3 \\
    \bottomrule
    \multicolumn{1}{c}{~} &
    \multicolumn{2}{c@{}}{\small{$\lfloor$ \hfill {\scriptsize term-weighting} \hfill $\rfloor$}} &
    \multicolumn{2}{c}{\small{$\lfloor$ \hfill {\scriptsize doc. expansion} \hfill $\rfloor$}}
    \end{tabular}
    \caption{Proportion of \underline{P}resent, \underline{R}eordered, \underline{M}ixed and \underline{U}nseen keyphrases in datasets. We also report the ratio of unique, unseen words in M+U keyphrases (\%uw).}
    \label{tab:datasets}
\end{table*}


==> tables/dist-model.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{clrrrr|r}
    %\multicolumn{3}{c}{~} &
    %\multicolumn{3}{c}{\small{$\lceil$ \hfill {\scriptsize absent keyphrases} \hfill $\rceil$}}
    \\
    \midrule
    \textbf{Model} & \textbf{Dataset} & \textbf{\%P} & \textbf{\%R} & \textbf{\%M} & \textbf{\%U} & \textbf{\%uw} \\
    \midrule
         %CopyRNN
         \multirow{2}{*}{\rotatebox{90}{seq2seq+copy}}
                 &    KP20k & 89.8 &  5.3 &  3.2 &  1.7 & 22.4 \\
                 & NTCIR1+2 & 96.9 &  1.3 &  0.9 &  0.9 & 12.3 \\
        \midrule
         %CorrRNN
         \multirow{2}{*}{\rotatebox{90}{seq2seq+corr}}
                 &    KP20k & 87.9 &  7.6 &  2.8 &  1.7 &  6.2 \\
                 & NTCIR1+2 & 89.7 &  7.1 &  2.5 &  0.8 &  3.2 \\
        \midrule
        %catTGNet
        \multirow{2}{*}{\rotatebox{90}{cat-seq2seq+tg}}
                 &    KP20k & 72.0 &  6.7 & 15.6 &  5.6 & 15.3 \\
                 & NTCIR1+2 & 52.3 &  3.0 &  8.7 & 36.0 & 40.0 \\
        \midrule
            gold
                 &    KP20k & 60.2 &  9.5 & 15.4 & 15.0 & 22.3 \\
                 & NTCIR1+2 & 61.2 &  8.2 & 16.6 & 14.1 & 21.5 \\
    \bottomrule
    %\multicolumn{2}{c}{~} &
    %\multicolumn{2}{c@{}}{\small{$\lfloor$ \hfill {\scriptsize term-weighting} \hfill $\rfloor$}} &
    %\multicolumn{2}{c}{\small{$\lfloor$ \hfill {\scriptsize doc. expansion} \hfill $\rfloor$}}
    \end{tabular}
    \caption{Proportion of \underline{P}resent, \underline{R}eordered, \underline{M}ixed and \underline{U}nseen keyphrases in top 10 model's output. We also report the ratio of unique, unseen words in M+U keyphrases (\%uw). \textcolor{purple}{C'est un très gros tableau, mais c'est juste pour le regarder.}}
    \label{tab:dist-model}
\end{table}


